GAMEOPT: Optimal Real-time Multi-Agent Planning and Control for Dynamic Intersections

We propose GameOpt: a novel hybrid approach to cooperative intersection control for dynamic, multi-lane, unsignalized intersections. Safely navigating these complex and accident prone intersections requires simultaneous trajectory planning and negotiation among drivers. GameOpt is a hybrid formulation that first uses an auction mechanism to generate a priority entrance sequence for every agent, followed by an optimization-based trajectory planner that computes velocity controls that satisfy the priority sequence. This coupling operates at real-time speeds of less than 10 milliseconds in high density traffic of more than 10,000 vehicles/hr, 100 times faster than other fully optimization-based methods, while providing guarantees in terms of fairness, safety, and efficiency. Tested on the SUMO simulator, our algorithm improves throughput by at least 25%, time taken to reach the goal by 75%, and fuel consumption by 33% compared to auction-based approaches and signaled approaches using traffic-lights and stop signs.

==> Sections/Theory.tex <==
\section{Analysis of different bidding strategies}
\label{sec: np-complete}
\input{Tables/comp_auctions}
\input{{Tables/accuracy}}

At this point, there are two concerns that may come to the mind of the reader:

\begin{enumerate}[noitemsep]
    \item Justification of using driver behavior as the bidding strategy as opposed to using monetary budgets, arrival times, or any random driver-specific property, \textit{e.g.} height.
    
    \item Since the optimal solution in \model~is to reward more aggressive drivers, conservative agents may be motivated to act aggressively.
\end{enumerate}

\noindent In the following, we formally address both issues.
% In Section~\ref{subsec: alternate_strat}, 

% we show that in economic auctions, random bidding (using arbitrary driver properties \textit{e.g.} height), and FIFO-based strategies, agents actually gain more utility by over-bidding implying that such auctions are not incentive-compatible whereas behavior-based bidding is game-theoretically optimal (Section~\ref{subsec: optimality}).

% In Section~\ref{subsec: behavior_and_conservative}, we provide an insight into why 

\subsection{Justifying behavior-based bidding for human drivers with social preferences}
\label{subsec: alternate_strat}

The key insight to achieving an optimal auction is that agents' bidding strategy ($\bm{b}$) should be correlated with their social preferences or private valuations ($\bm{v}$). That is,

\begin{equation}
\begin{split}
    \bm{b}_1 > \bm{b}_2& > \ldots > \bm{b}_K\\
    &\iff\\
    \bm{v}_1 > \bm{v}_2& > \ldots > \bm{v}_K\\
\end{split}
\end{equation}

\noindent \hllb{where $\iff$ denotes equivalency} and with optimality occurring when $\bm{b}_i = \bm{v}_i = \bm{\zeta}_i$. In the case of behavior-based bidding, we explicitly enforce the above constraints via \model. Economic auctions, random bidding, and FIFO-based strategies, on the other hand, disregard the aspect of human social preference ($\bm{v}$). A simple analysis reveals that ignoring private valuations can result in auctions where agents are encouraged to falsify their bids.

% As before, let $\bm{b}_1 > \bm{b}_2 > \ldots > \bm{b}_K$ and $\bm{\alpha}_1 > \bm{\alpha}_2 > \ldots > \bm{\alpha}_K$ denote the order of bids and associated time-rewards for agents $a_1, a_2, \ldots, a_K$. The nature of bids depend on the particular mechanism; they represent money in the case of economic auctions and time-to-intersection (or roundabout) in the case of FIFO-based auctions.
Consider any economic auction~\cite{carlino2013auction}. Let the cash bids made by agents be $\bm{b}_1 > \bm{b}_2 > \ldots > \bm{b}_K$ with associated time rewards, $\bm{\alpha}_1 > \bm{\alpha}_2 > \ldots > \bm{\alpha}_K$. Now assume a single agent $a_k$ is an impatient driver with a budget $B_k$ and bid $\bm{b}_k \leq B_k$ ($B_k < B_m$ where $m$ indexes those agents whose bid $\bm{b}_m > \bm{b}_k$). Since economic auctions do not take social preferences or private valuations into account, it can be shown that $\bm{v}_k > \bm{b}_k$ for the impatient agent $a_k$. To see how, recall that $a_k$'s private valuation $\bm{v}_k$ is much higher than the agents before them. That is, $\exists m<k$ such that $\bm{v}_k > \bm{v}_m$. Without loss of generality, assume $m=k-1$. Then we have that $\bm{v}_1 > \ldots>\bm{v}_k> \bm{v}_{k-1}>\ldots> \bm{v}_K$. Since $\bm{v}_k>\bm{v}_{k-1}$ but $\bm{b}_{k-1}>\bm{b}_k$ and $\bm{v}_{k-1} = \bm{b}_{k-1}$, $\bm{v}_k > \bm{b}_{k}$ and $a_k$ can decide to increase her bid to $\bm{\bar b}_k = \bm{b}_{k-1} + \epsilon >\bm{b}_{k-1}$. The updated utility for $a_k$ is,

\begin{equation*}
% \begin{split}
    \bm{\bar u}_k (\bm{\bar b}_k) = \bm{v}_k \left( \frac{1}{t_{k-1}} \right ) - \sum_{j=k-1}^K \bm{b}_{j+1} \left(\frac{1}{t_j} - \frac{1}{t_{j+1}} \right).
% \end{split}    
\end{equation*}

\noindent The difference from original utility is,

\begin{equation}
% \begin{split}
    % &\bar u_k (\bar \bm{b}_k) = \\
    \bm{d} = \left( \bm{v}_k - \bm{b}_k \right)  \left( \frac{1}{t_{k-1}} - \frac{1}{t_{k}} \right ).
    \label{eq: difference}
% \end{split}    
\end{equation}
    

\noindent Since $\bm{v}_k > \bm{b}_k$ and $t_{k-1} < t_{k}$, the net change is positive. Therefore, agents gain utility by over-bidding. This implies that economic and FIFO-based auctions are not optimal. We present empirical evidence in Section~\ref{subsec: comparison_with_prior_methods}.


\subsection{Behavior-based bidding does not encourage conservative agents to act aggressively}
\label{subsec: behavior_and_conservative}
At first glance, it may seem that a similar argument can be made against our approach wherein it is biased towards aggressive drivers by rewarding them with higher priority, thereby encouraging conservative drivers to be more aggressive (over-bidding). However, this is not the case since in the case of behavior-based bidding, acting aggressively and therefore, over-bidding $\bm{b}_k > \bm{v}_k \implies \bm{d} < 0$ by Equation~\ref{eq: difference}. In other words, conservative drivers lose utility by acting aggressively. \hllg{This is because in the event of an overbid, the gain in time reward, $\bm{\zeta}_{k}\left( \frac{1}{t_{k-1}} - \frac{1}{t_{k}}\right)$ is \textit{less} than the risk penalty, $\bm{b}_{k}\left( \frac{1}{t_{k-1}} - \frac{1}{t_{k}}\right)$. Special cases include when two or more agents decide to over bid at the same time. The driver behavior modeling algorithm, CMetric, automatically takes care of these issues as it outputs a real number ($\mathbb{R}$). In the unlikely event that the CMetric output for multiple vehicles be identical, we choose to break ties randomly.}


==> Sections/back.tex <==
\section{Background and Problem Formulation}
In this section, we begin by defining several key terms and stating the problem statement followed by the assumptions made in our approach. We briefly summarize the CMetric algorithm~\cite{cmetric} for behavior modeling and prediction and provide an overview on sponsored search auctions~\cite{roughgarden2016twenty}, which are widely used in game theory.

\subsection{Problem formulation}
\label{subsec: problem_formulation}

We frame navigating unsignaled intersections, roundabouts, and merging scenarios as a multi-agent game-theoretic non-sequential decision-making problem. We consider three unsignaled and uncontrolled traffic scenarios or environments -- intersections, merging, and roundabouts with multiple non-communicating human drivers and AVs. In each of the three scenarios, we refer to a traffic-agent as ``active'' if they participate in the decision-making process for navigating the scenario. For example, the lead traffic-agents in each service lane of a four-way intersection are active vehicles, while agents waiting in line behind their respective lead vehicle are non-active agents. We denote the active agents as a set $\mathcal{A} = \{a_1, a_2, \ldots a_n \}$. The action space for each active agent is a discrete set consisting of finite acceleration values. The state space consists of the position $x_t \in \mathcal{X}$ and velocity $v_t$ of each agent measured in a global coordinate frame (\textit{e.g.} GPS coordinates or $3-$D points obtained using GPS and lidars, respectively).

\subsection{Modeling human driver behavior}
\label{subsec: cmetric_background}

Each active agent is characterized by a behavior profile, $\bm{\zeta}_i$, which can be obtained via recent behavior modeling algorithms such as the SVO~\cite{schwarting2019social} and CMetric~\cite{cmetric}. In this work, we use CMetric to quantify the aggressiveness or conservativeness of a traffic-agent. This model provides an objective measure of aggressiveness based on driving maneuvers such as overspeeding, overtaking and so on. We briefly summarize the CMetric algorithm. To determine if an agent is aggressive or conservative, the algorithm begins by reading the trajectories of the ego-agent and surrounding vehicles via cameras or lidars during any time-period $\Delta t$. The trajectory of an agent is represented by 

\[\Xi_{\Delta t} = \{x_t \ | \ t = t_0, t_1, \ldots, t_0 + \Delta t \}.\]

\noindent In CMetric, these trajectories are represented via weighted undirected graphs $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ in which the vertices denote the positions for each agent and the edges correspond to the distances between agents. The algorithm proceeds by using these graphs to model the likelihood and intensity of driving behavior indicators like overspeeding, overtaking, sudden ``zig-zagging'' and lane-changes via centrality functions~\cite{rodrigues2019network} represented by $\Phi: \mathcal{G}\rightarrow \mathbb{R}$. These behavior indicators determine whether an agent is aggressive or conservative~\cite{sagberg2015review}. The behavior profile for $a_i$ is denoted by $\bm{\zeta}_i$ and can be computed using,

\begin{equation}
    \bm{\zeta}_i(\Xi_{\Delta t}) = \Phi(\mathcal{G}),
    \label{eq: cmetric}
\end{equation}

\noindent where $\mathcal{G}(\mathcal{V}, \mathcal{E})$ is constructed using $\Xi_{\Delta t}$. In this work, we use CMetric to compute the behavior profiles of traffic-agents, represented by a $n-$dimensional vector $\bm{\zeta},$ that is provided to the auction program.

\subsection{Assumptions}
\label{subsec: assumptions}

We assume agents (AVs and human drivers) are rational and strive to maximize their own utility which can be independent of other agents. Further, agents are \textit{non-ideal} (in contrast to ideal agents in~\cite{cleac2020lucidgames, cleac2019algames, wang2020game}) in that they do not have access to the actions, objectives, or utility functions of other agents. We make no assumptions on the motion or dynamics of traffic-agents. The state-space is fully observable by all agents (active and non-active). We assume the availability of a behavior modeling and prediction algorithm such as CMetric~\cite{cmetric} that models driving behavior as being either aggressive or conservative. This information is provided to an auction program. We assume that agents navigate through the environment one at a time and do not use traffic signals, employ right-of-way rules, or communicate with other agents.

\subsection{Sponsored search auctions (SSAs)}
\label{subsec: SSA_background}
Sponsored search auctions (SSAs) are a game-theoretic mechanism that are used extensively in internet search engines for the purpose of internet advertising~\cite{roughgarden2016twenty}. In an SSA, there are $K$ items to be allocated among $n$ agents. Each agent $a_i$ has a private valuation $\bm{v}_i$ and submits a bid $\bm{b}_i$ to receive at most one item of value $\bm{\alpha}_i$. A strategy is defined as an $n$ dimensional vector, $\bm{b} = (\bm{b}_i \cup \bm{b}_{-i})$, representing the bids made by every agent. $\bm{b}_{-i})$ denotes the bids made by all agents except $a_i$. Furthermore, let $\bm{b}_1 > \bm{b}_2 > \ldots > \bm{b}_K$ and $\bm{\alpha}_1 > \bm{\alpha}_2 > \ldots > \bm{\alpha}_K$. The allocation rule is that the agent with the $i^\textrm{th}$ highest bid is allocated the $i^\textrm{th}$ most valuable item, $\bm{\alpha}_i$. The utility $\bm{u}_i$~\cite{roughgarden2016twenty} incurred by $a_i$ is given as follows,

\begin{equation}
 \bm{u}_i (\bm{b}_i) =  \bm{v}_i \bm{\alpha}_i - \sum_{j=i}^k \bm{b}_{j+1} \left( \bm{\alpha}_j - \bm{\alpha}_{j+1} \right).
 \label{eq: utility_template}
\end{equation}

\noindent In the equation above, the quantity on the left represents the total utility for $a_i$ which is equal to value of the allocated goods $\bm{\alpha}_i$ minus a payment term. The first term on the right is the value of the item obtained by $a_i$. The second term on the right is the payment made by $a_i$ as a function of bids $\bm{b}_{j > i}$ and their allocated item values $\bm{\alpha}_j$. We refer the reader to Chapter $3$ in~\cite{roughgarden2016twenty} for a derivation and detailed analysis of Equation~\ref{eq: utility_template}.

In our approach, we re-cast Equation~\ref{eq: utility_template} through the lens of a human driver. More specifically, the term $\bm{v}_i \bm{\alpha}_i$ denotes the time reward gained by driver $a_i$ by moving on her turn. The payment term represents a notion of risk~\cite{wang2020game} associated with moving on that turn. It follows that an allocation of a conservative agent to a later turn (smaller $\bm{\alpha}$) also presents the lowest risk and vice-versa.

\subsection{Problem statement}

To prevent collisions and deadlocks, it is necessary to determine the order in which agents take turns to navigate the traffic scenario~\cite{carlino2013auction, dresner2008multiagent, lin2021pay, sayin2018information, schepperle2007agent, vasirani2012market}. Thus, the goal of this paper (formalized shortly via Problem~\ref{problem: prob}) is to compute an optimal turn-based ordering which is defined as follows,

% \input{NeuRIPS2020/img/overview/overview}

\begin{definition}
\textbf{Turn-based Orderings ($\bm{\sigma}$): } A turn-based ordering is a permutation $\bm{\sigma}: \mathcal{A} \rightarrow [1,n]$ over the set $\mathcal{A}$. For any $i,j \in [1,n]$, $\bm{\sigma}(a_i) = j$, equivalently $\bm{\sigma}_i = j$, indicates that $a_i$ with driving behavior $\bm{\zeta}_i$ will move on the $j^\textrm{th}$ turn.
\label{def: turn_based_ordering}
\end{definition}


\noindent There may be multiple turn-based orderings that may apply in a given scenario. However, many of them could be sub-optimal and may result in collisions and deadlocks. An optimal turn-based ordering prevents collisions and resolves deadlock conflicts.

\begin{definition}
\textbf{Optimal Turn-based Ordering ($\bm{\sigma}_{\textsc{opt}}$): } A turn-based ordering, $\bm{\sigma}$, over a given set $\mathcal{A}$ is game-theoretically optimal if it is incentive compatible, welfare maximizing, and can be computed in polynomial time\footnote{These terms are defined in Section~\ref{subsec: optimality}}.
\label{def: optimal_turn_based_ordering}
\end{definition}

\noindent We now ready to formally state our goal in this paper as follows,

\begin{problem}
In a traffic scenario (which could be an intersection, roundabout, or merging) with $n$ active road-agents, given the behavior profile $\bm{\zeta}_i$ of each agent, the goal is to compute the optimal turn-based ordering $\bm{\sigma}_\textsc{opt}  = \bm{\sigma}_1\bm{\sigma}_2\ldots\bm{\sigma}_n$.
\label{problem: prob}
\end{problem}


% \input{NeuRIPS2020/img/overview/overview}
% In game theory, a strategy is defined as an $n$ dimensional vector, $b = (\bm{b}_i \cup \bm{b}_{-i})$, representing the bids made by every agent. The goal of any optimal auction is to generate maximum welfare upon truthful bidding so that that no agent is incentivised to ``cheat'' \textit{i.e.} incentive compatible. In other words, auctions are incentive compatible when the dominant strategy for each agent is to bid their true valuation $v_i$.
% In our proposed approach, we combine the SSA with the CMetric behavior modeling algorithm to generate an auction with a novel bidding strategy. We discuss this approach in detail in the following section. 
% We conclude current section with the some standard, but important, definitions related to game-theoretic optimality.

% \begin{definition}
% \textbf{Dominant Strategy:} Bidding $\bm{b}_i$ is a dominant strategy for $a_i$ if $\bm{u}_i(\bm{b}_i, \bar \bm{b}_{-i}) > \bm{u}_i(\bar \bm{b}_i, \bar \bm{b}_{-i})$ for all $\bar \bm{b}_i \neq \bm{b}_i$.
% \end{definition}

% We now state two important definitions that are used as the basis of an optimal SSA.

% \begin{definition}
% \textbf{Incentive Compatibility:} An auction is said to be incentive compatible if for each agent, bidding $\bm{b}_i = v_i$ is a dominant strategy.
% \label{def: incentive_compatibility}
% \end{definition}

% \begin{definition}
% \textbf{Welfare Maximization:} Social welfare of an auction outcome is defined as $\sum_i v_i \bm{u}_i(\bm{b}_i)$. Welfare maximization is the task of finding the strategy $b$ that maximizes $\sum_i v_i \bm{u}_i(\bm{b}_i)$.
% \label{def: social_welfare}
% \end{definition}

% Finally, SSAs have polynomial time complexity since sorting is polynomial time~\cite{clrs}.
% \subsubsection{Sponsored Search Auctions}

% \subsubsection{Optimality and Efficiency of SSAs}




==> Tables/accuracy.tex <==
\begin{table}[t]
% \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
\caption{\textbf{Comparing with other approaches:} We compare the percentage \hllb{(\%)} of collisions (C), deadlocks (D), and overall success rate (S) with state-of-the-art planning methods designed for uncontrolled and unsignaled intersections. The \xmark~symbol indicates that results for that setting were not provided by the method.
}
\centering
% \setlength{\tabcolsep}{3mm}
% \ra{1.05}
% \Large
% \begin{adjustbox}{max width=\textwidth}
\resizebox{\columnwidth}{!}{
\begin{tabular}{rccccccccc}
  \toprule[1.5pt]
%   \multirow{4}[3]{*}{Methods}&&&&$4-$way intersection&&&&&\\ 
%   \cmidrule[1pt](l{3mm}r{3mm}){3-13}   &
% \midrule
 \multirow{2}{*}{Methods}& \multicolumn{3}{c}{$2$ Vehicles} &
  \multicolumn{3}{c}{$3$ Vehicles}&  
  \multicolumn{3}{c}{$4$ Vehicles}\\
%   \cmidrule{3-5} 
%   \cmidrule(l{3mm}r{3mm}){7-9} 
%   \cmidrule(l{3mm}r{3mm}){11-13}
   & {C } & {D } & S  &  {C } & {D } & S  &  {C } & {D } & S \\
%   \midrule
%   \midrule
\midrule
%  &&&&&&$4-$way Intersection Groups&&&&&&\\ 
%   \midrule

  Capasso et al.~\cite{capasso2021end} & 
    \xmark & \xmark & \xmark & 
    $02$ & \xmark & \xmark & 
    $0$ & \xmark & \xmark  \\ 
  Liu et al.~\cite{liu2020decision} & 
    \xmark & \xmark & \xmark & 
    \xmark & \xmark & \xmark & 
    $6.2$ & \xmark & $93.7$  \\ 
  Isele et al.~\cite{isele2018navigating} & 
    \xmark & \xmark & \xmark & 
    \xmark & \xmark & \xmark & 
    $7.1$ & $0.2$ & $92.8$  \\ 
Kai et al.~\cite{Kai2020AMR} & 
    $0$ & $0$ & $100$ & 
    \xmark & \xmark & \xmark & 
    $3.7$ & $0 $ & $96.3$  \\ 
    
  Li et al.~\cite{li2020game} & 
    $0$ & $0$ & $100$ & 
    \xmark & \xmark & \xmark & 
    $2.7$ & $0.4$ & $96.9$  \\ 
  Roh et al.~\cite{roh2020multimodal} &
    $2$ & \xmark & $98$& $2$ & \xmark & $98$ & $30$ & \xmark & $70$   \\ 
  Tian et al.~\cite{tian2020game} &
    $10$ & $5$ & $85$ & 
    $10$ & $5$ & $85$ & 
    $10$ & $10$ & $80$  \\ 
  \model  & 
    $\textbf{0}$ & $\textbf{0}$ & $\textbf{100}$ & 
    $\textbf{0}$ & $\textbf{0}$ & $\textbf{100}$ & 
    $\textbf{0.1}$ & $\textbf{0.1}$ & $\textbf{99.8}$  \\ 
  \midrule
  
%  \midrule
%   \midrule
%     \multirow{4}[3]{*}{Methods}&&&&$ 4-$way intersection&&&&&\\ 
%   \midrule
  \multirow{2}{*}{Methods}&
  \multicolumn{3}{c}{$6$ Vehicles}& 
  \multicolumn{3}{c}{$8$ Vehicles}&  
  \multicolumn{3}{c}{$10$ Vehicles}\\
%   \cmidrule(l{3mm}r{3mm}){3-5} 
%   \cmidrule(l{3mm}r{3mm}){7-9} 
%   \cmidrule(l{3mm}r{3mm}){11-13}
   & {C } & {D } & S  &  {C } & {D } & S  &  {C } & {D } & S \\
  \midrule
    Capasso et al.~\cite{capasso2021end} & 
    \xmark & \xmark & \xmark &
    $03$ & \xmark & \xmark &
    \xmark & \xmark & \xmark  \\
  Li et al.~\cite{li2020game} &
    $10$ & $10$ & $90$ &
    $20$ & $20$ & $80$ &
    $20$ & $20$ & $80$  \\ 
  Tian et al.~\cite{tian2020game} &
    $10$ & $10$ & $80$ &
    $10$ & $10$ & $80$ &
    $20$ & $20$ & $60$  \\ 
    
    \midrule
  \model  &
    $\textbf{0.3}$ & $\textbf{0.1}$ & $\textbf{99.6}$ &
    $\textbf{0.4}$ & $\textbf{0.1}$ & $\textbf{99.5}$ &
    $\textbf{0.6}$ & $\textbf{0.2}$ & $\textbf{99.2}$  \\ 


  \bottomrule[1.5pt]
\end{tabular}
}
% \end{adjustbox}
% \vspace{-6mm}
\label{tab: accuracy}
  \vspace{-10pt}
 
\end{table}

==> Tables/benefits.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Benefits of \model~over prior work in planning.}}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}

\toprule
%  &  &  & \multicolumn{2}{c}{Our CMetric Measures}\\

% \cline{4-5}
Problem Setting & Approach & Methods & Assumptions/Limitations & Benefits\\
\midrule
\multirow{2}{*}{Single-agent planning with dynamic obstacles} & Geometric Methods  && \\
                                             & Learning-based Methods && \\


\multirow{2}{*}{Multi-agent planning} & Game theory  && \\
                                             & Auctions && \\
 
\bottomrule
\end{tabular}
}
\label{tab: benefits}

\end{table*}

==> Tables/bidding.tex <==
\begin{table}%[tbhp]
\centering
\caption{\textbf{Summary of prior work:} We list methods for navigating unsignaled intersections, roundabouts, and merging based on multi-agent planning (MAP), action space (AS), and incentive compatibility (IC). \cmark$^{*}$ corresponding to a method indicates that optimality does not hold for human drivers with varying social preferences.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrccccc}
\toprule
Approach & Methods & Optimality & Multi-Agent & Planner & Cost & Dynamic\\
\midrule
\multirow{4}{*}{\small DRL}& Capasso et al.~\cite{capasso2021end} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark &C & -& \cellcolor{red!25} \xmark\\
& Isele et al.~\cite{isele2018navigating} &\cellcolor{red!25} \xmark&\cellcolor{red!25} \xmark&D & -& \cellcolor{red!25} \xmark\\
& Kai et al.~\cite{Kai2020AMR} &\cellcolor{red!25} \xmark&\cellcolor{red!25} \xmark& D & -& \cellcolor{green!25} \cmark\\
& Liu et al.~\cite{liu2020decision} &\cellcolor{red!25} \xmark&\cellcolor{red!25} \xmark&D & -& \cellcolor{red!25} \xmark\\
\cmidrule{2-7}

\multirow{2}{*}{\small Game Theory}& Li et al.~\cite{li2020game} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&C & -& \cellcolor{red!25} \xmark\\
& Tian et al.~\cite{tian2020game} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&C & -& \cellcolor{red!25} \xmark\\
\cmidrule{2-7}

{RNN} & Roh et al.~\cite{roh2020multimodal} &\cellcolor{red!25} \xmark&\cellcolor{red!25} \xmark&C & -& \cellcolor{red!25} \xmark\\
\cmidrule{2-7}

% \multirow{2}{*}{\small FIFO}& FIFO (basic) &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
% & Buckman et al.~\cite{gt6} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
% \cmidrule{2-8}

\multirow{8}{*}{\small Auctions}& FIFO &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
& Buckman et al.~\cite{gt6} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
& Vasirani and Ossowski~\cite{vasirani2012market}&\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & \cellcolor{red!25} \xmark& \cellcolor{red!25} \xmark\\
& Censi et al.~\cite{censi2019today}&\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & \cellcolor{red!25} \xmark& \cellcolor{red!25} \xmark\\
& Lin and Jabari~\cite{lin2021pay}&\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & \cellcolor{red!25} \xmark& \cellcolor{red!25} \xmark\\
& Carlino et al.~\cite{carlino2013auction} &\cellcolor{green!25} \cmark$^{*}$&\cellcolor{green!25} \cmark&D & \cellcolor{green!25} \cmark& \cellcolor{red!25} \xmark\\
& Rey et al.~\cite{rey2021online}&\cellcolor{green!25} \cmark$^{*}$&\cellcolor{green!25} \cmark&D & \cellcolor{green!25} \cmark& \cellcolor{green!25} \cmark\\
& Sayin et al.~\cite{sayin2018information} &\cellcolor{green!25} \cmark$^{*}$&\cellcolor{green!25} \cmark&D & \cellcolor{green!25} \cmark& \cellcolor{red!25} \xmark\\
& Chandra and Manocha~\cite{chandra2022gameplan} &\cellcolor{green!25} \cmark&\cellcolor{green!25} \cmark&High & \cellcolor{green!25} \cmark & \cellcolor{red!25} \xmark\\
\cmidrule{2-7}
& \textbf{This work} &\cellcolor{green!25} \cmark&\cellcolor{green!25} \cmark&Hybrid & \cellcolor{green!25} \cmark & \cellcolor{green!25} \cmark\\

\multirow{1}{*}{\small Optimization}& Suriyarachchi et al.~\cite{suriyarachchi2021real} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
& Buckman et al.~\cite{gt6} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
& Vasirani and Ossowski~\cite{vasirani2012market}&\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & \cellcolor{red!25} \xmark& \cellcolor{red!25} \xmark\\



\bottomrule
\end{tabular}
}
\label{tab: bidding_rules}
\vspace{-10pt}
% \addtabletext{nomenclature for the TSs refers to the numbered species in the table.}
\end{table}

\input{Tables/high_vs_low}

==> Tables/comp_auctions.tex <==
\begin{table*}[t]
{\fontsize{9pt}{9pt}\selectfont
% \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
\caption{\textbf{Using different bidding strategies:} We compare the rate of collisions by replacing the CMetric bidding strategy with economic auctions, first-in-first-out (FIFO), and random bidding in a range of simulation settings that include changing the traffic density, number of aggressive drivers, likelihood of a driver being aggressive, and speed limit.}
\label{tab: auctions}
\centering
% \setlength{\tabcolsep}{3mm}
% \ra{1.05}
% \Large
% \begin{adjustbox}{max width=\textwidth}
\fontsize{8}{10}\selectfont{\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccccc|cc|cccc|cc@{}}
  \toprule
%   \multirow{4}[2]{*}{Methods}&&&&&&$4-$way Intersection&&&&&&\\ 
%   \cmidrule[1pt](l{3mm}r{3mm}){3-17
%   } 
  \multirow{2}{*}{Strategy} &
  \multicolumn{4}{c}{\% Aggressive}&
  \multicolumn{2}{c}{\# Agg. Agents}& 
  \multicolumn{4}{c}{\# Agents \fontsize{7}{8}\selectfont{(w. 1 agg. agent)}} & 
  \multicolumn{2}{c}{Max. Speed} \\
  \cmidrule{2-5} 
  \cmidrule{6-7} 
  \cmidrule{8-11}
  \cmidrule{12-13}
   & $20\%$ & $25\%$ & $33\%$ & $50\%$ &  $1$ & $2$  &  $4$ & $6$ & $8$ & $10$ & $45$mph & $60$mph \\
%   \midrule
%   \midrule
\midrule
%  &&&&&&$4-$way Intersection Groups&&&&&&\\ 
%   \midrule

  Economic & 
    $2.48$ & $2.99$ & $6.55$ &
    $8.29$& $2.81$ & $6.18$ & 
    $3.07$ & $3.27$ & $3.58$ & $3.62$ &$2.99$& $3.07$ \\ 
  FIFO & 
    $7.18$ & $8.69$ & $10.20$ & 
    $15.87$& $7.65$ & $15.06$ & 
    $7.59$ & $8.36$ & $8.65$ & $8.91$ & $7.72$ & $7.47$ \\ 
  Random  & 
    $14.79$ & $18.67$ & $25.24$ &
    $37.77$ & $15.01$ & $28.91$ & 
    $14.82$ & $16.69$ & $17.59$  & $17.90$& $15.01$&$15.01$\\ 
  \textbf{\model}  & 
     $\textbf{0.33}$ & $\textbf{0.37}$ & $\textbf{0.63}$ & 
    $\textbf{0.79}$& $\textbf{0.29}$ & $\textbf{0.66}$ & 
    $\textbf{0.12}$ & $\textbf{0.24}$ & $\textbf{0.37}$  & $\textbf{0.64}$& $\textbf{0.44}$&$\textbf{0.53}$\\ 

  \bottomrule
\end{tabular}}
}
}
% \end{adjustbox}
% \vspace{-6mm}
  \vspace{-5pt}
\end{table*}

==> Tables/notation.tex <==
\begin{table}[t]
  \caption{Symbols and notations used in this paper.}
  \label{tab: notation}
  \centering
  \resizebox{.7\columnwidth}{!}{%
  \begin{wraptable}{r}{5.5cm}
  \begin{tabular}{cl}
  \toprule
    Symbol  & Description \\
    \midrule
    $n$ & Number of traffic-agents.\\
    $a_i$ & $i^\textrm{th}$ active agent.\\
    $\mathcal{A}$ & Set of active agents. \\
    $\zeta$ & CMetric-based behavior profile (Section~\ref{subsec: cmetric_background}). \\
    $\sigma$ & Turn-based ordering (Definition~\ref{def: turn_based_ordering}). \\
    $\sigma_{\textsc{opt}}$ & Optimal turn-based ordering (Definition~\ref{def: optimal_turn_based_ordering}). \\
    $b_i$ & Bid of the $i^\textrm{th}$ active agent.\\
    $b_{-i}$ & Bid of every agent except the $i^\textrm{th}$.\\
    $v_i$ & Private valuation of the $i^\textrm{th}$ active agent.\\
    $u_i(\cdot)$ & Utility of the $i^\textrm{th}$ active agent.\\
    $t_i$ & Time taken by the $i^\textrm{th}$ active agent \\
    & to navigate the traffic scenario.\\

    \bottomrule
  \end{tabular}
  \end{wraptable} 
  }
%   }
  \vspace{-15pt}
\end{table}


==> Tables/parameters.tex <==
\begin{table}[h]
\caption{IDM and MOBIL parameters used for Conservative and Aggressive vehicle classes}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{clcc} 
\toprule
Model & Parameter \Tstrut & Conservative \Bstrut &   Aggressive \\
\hline
\multirow{4}{*}{IDM}& Time gap ( $T$) \Tstrut & 1.5s      & 1.2s \\
 &Min distance ($s_0$) & 5.0 $m$ & 2.5 $m$ \\
&Max comfort acc. ($a$)     & 3.0 $m/s^2$ & 6.0 $m/s^2$\\
&Max comfort dec. ($b$) & 6.0 $m/s^2$               &  9.0 $m/s^2$ \\
\midrule
\multirow{3}{*}{MOBIL}& Politeness ($p$) & 0.5     & 0\\
& Min acc gain ($\Delta a_{th}$) & 0.2 $m/s^2$ & 0 $m/s^2$ \\
& Safe acc limit ($b_{safe}$) & 3.0 $m/s^2$ & 9.0 $m/s^2$\\
\bottomrule
\end{tabular}
}
\label{tab: parameters}
\vspace{-10pt}
\end{table}

